Fractional statistical dynamics and fractional kinetics

We apply the subordination principle to construct kinetic fractional statistical dynamics in the continuum in terms of solutions to Vlasov-type hierarchies. As a by-product we obtain the evolution of the density of particles in the fractional kinetics in terms of a non-linear Vlasov-type kinetic equation. As an application we study the intermittency of the fractional mesoscopic dynamics.

==> jinfo.tex <==
\jvolume{22}
\jyear{2016}
\jnumber{3}

